NECA: Neural Customizable Human Avatar

Human avatar has become a novel type of 3D asset with various applications. Ideally, a human avatar should be fully customizable to accommodate different settings and environments. In this work, we introduce NECA, an approach capable of learning versatile human representation from monocular or sparse-view videos, enabling granular customization across aspects such as pose, shadow, shape, lighting and texture. The core of our approach is to represent humans in complementary dual spaces and predict disentangled neural fields of geometry, albedo, shadow, as well as an external lighting, from which we are able to derive realistic rendering with high-frequency details via volumetric rendering. Extensive experiments demonstrate the advantage of our method over the state-of-the-art methods in photorealistic rendering, as well as various editing tasks such as novel pose synthesis and relighting. The code is available at https://github.com/iSEE-Laboratory/NECA.

==> figs/shadow_trans.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/rebuttal/shadow/shadow_trans.pdf}
    \vspace{-3mm}
\caption{\textbf{Results of shadow transfer.}}
\vspace{-8mm}
\label{fig:shadow_trans}
\end{figure}

==> figs/syn_dataset.tex <==
\begin{figure}[t]  
  \centering            
  \subfloat
  {
   \includegraphics[width=0.3\linewidth]{figs/syn_dataset/eric_cave.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/eric_brown.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/eric_night.png}
  }
\vspace{1mm}
  \subfloat
  {
   \includegraphics[width=0.3\linewidth]{figs/syn_dataset/carla_cave.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/carla_brown.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/carla_night.png}
  }
\vspace{1mm}
  \subfloat
  {
   \includegraphics[width=0.3\linewidth]{figs/syn_dataset/claudia_cave.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/claudia_brown.png}
  }
  \subfloat
  {
      \includegraphics[width=0.3\linewidth]{figs/syn_dataset/claudia_night.png}
  }
   
 \caption{\textbf{Visualization of Synthetic Dataset.} Each row we show the 3D human character under different HDRI maps. }

\label{fig:syn_dataset}
\end{figure}

==> figs/video_failure.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{figs/rebuttal/video_comparison.pdf}
    \vspace{-7mm}
\caption{\textbf{Video comparison with PV on the subjects in Fig. 4 in the paper.} We show several frames of each video here. The complete video results will be included in the supplementary material.}
\vspace{-5mm}
\label{fig:video}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/novel_pose.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l  c  c c  c  c  c  c  c  c}
\toprule[1pt]
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{313} & \multicolumn{3}{c}{315} & \multicolumn{3}{c}{377} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& 24.1 & 0.908 & 0.126
& 19.8 & 0.867 & 0.152 
& 24.2 & 0.917 & 0.119 \\
AN~\cite{peng2021animatable} 
& 23.9 & 0.909 & 0.115 
& 19.2 & 0.855 & 0.167 
& 22.6 & 0.900 & 0.153 \\
DS~\cite{zhi2022dual} 
& 24.3 & 0.909 & 0.110 
& 19.5 & 0.861 & 0.166 
& 24.7 & 0.919 & 0.137 \\
ARAH~\cite{ARAH:2022:ECCV} 
& 24.4 & 0.914 & 0.092 
& 20.0 & 0.881 & 0.105 
& 25.5 & 0.933 & 0.093 \\
PV~\cite{li2023posevocab} 
& 23.9 & 0.911 & 0.085 
& 20.2 & 0.869 & 0.106 
& 24.8 & 0.925 & 0.074 \\
Ours & \textbf{24.7}  & \textbf{0.919} & \textbf{0.082}
& \textbf{20.8}  & \textbf{0.884} & \textbf{0.101}
& \textbf{26.3} & \textbf{0.939} & \textbf{0.066} \\
\midrule
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{386} & \multicolumn{3}{c}{387} & \multicolumn{3}{c}{390} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& 26.1 & 0.894 & 0.171 
& 21.4 & 0.865 & 0.160 
& 24.2 & 0.882 & 0.164 \\
AN~\cite{peng2021animatable} 
& 25.5 & 0.884 & 0.187 
& 21.4 & 0.868 & 0.169
& 23.9 & 0.887 & 0.173 \\
DS~\cite{zhi2022dual} 
& 26.0 & 0.888 & 0.171 
& 22.4 & 0.880 & 0.180 
& 23.7 & 0.877 & 0.195 \\
ARAH~\cite{ARAH:2022:ECCV} 
& 27.0 & 0.910 & 0.127 
& 23.5 & 0.901 & 0.113 
& 24.8 & 0.896 & 0.126 \\
PV~\cite{li2023posevocab} 
& 27.3 & 0.913 & \textbf{0.101} 
& 23.4 & 0.898 & 0.103 
& 24.6 & 0.895 & 0.114 \\
Ours & \textbf{27.5}  & \textbf{0.916} & 0.103
& \textbf{23.9}  & \textbf{0.907} & \textbf{0.098}
& \textbf{25.2} & \textbf{0.905} & \textbf{0.106} \\
\midrule
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{392} & \multicolumn{3}{c}{393} & \multicolumn{3}{c}{394} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& 26.0 & 0.916 & 0.135 
& 23.5 & 0.900 & 0.132 
& 24.1 & 0.888 & 0.150 \\
AN~\cite{peng2021animatable} 
& 24.3 & 0.900 & 0.169 
& 23.8 & 0.897 & 0.155 
& 24.1 & 0.887 & 0.171 \\
DS~\cite{zhi2022dual} 
& 25.8 & 0.914 & 0.144 
& 23.2 & 0.894 & 0.147 
& 24.3 & 0.888 & 0.163 \\
ARAH~\cite{ARAH:2022:ECCV} 
& 26.2 & 0.927 & 0.106 
& 24.4 & 0.915 & 0.104 
& 25.2 & 0.908 & 0.111 \\
PV~\cite{li2023posevocab} 
& 25.4 & 0.920 & 0.089 
& 24.1 & 0.910 & \textbf{0.089} 
& 24.6 & 0.902 & 0.093 \\
Ours & \textbf{26.8}  & \textbf{0.932} & \textbf{0.084}
& \textbf{24.8}  & \textbf{0.919} & 0.090
& \textbf{25.3} & \textbf{0.909} & \textbf{0.092 } \\
\bottomrule[1pt]
\end{tabular}
}
\caption{\textbf{Novel pose synthesis quantitative comparison on ZJU-MoCap dataset.} We show the results of each subject.}
\label{table:detail_np}
\end{table*}

==> tables/novel_view.tex <==
\begin{table*}[t]
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{l  c  c c  c  c  c  c  c  c}
\toprule[1pt]
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{313} & \multicolumn{3}{c}{315} & \multicolumn{3}{c}{377} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& 30.5 & 0.967 & 0.068 
& 26.4 & 0.958 & 0.079 
& 28.1 & 0.956 & 0.080 \\
AN~\cite{peng2021animatable} 
& 29.8 & 0.963 & 0.075 
& 23.1 & 0.917 & 0.138 
& 24.2 & 0.925 & 0.124 \\
DS~\cite{zhi2022dual} 
& \textbf{31.6} & 0.972 & 0.067 
& 25.8 & 0.950 & 0.116 
& 27.3 & 0.949 & 0.105 \\
ARAH~\cite{ARAH:2022:ECCV} 
& \textbf{31.6} & 0.973 & 0.050 
& \textbf{27.0} & \textbf{0.965} & 0.058 
& 27.8 & \textbf{0.956} & 0.071 \\
PV~\cite{li2023posevocab} 
& 30.2 & 0.968 & 0.038 
& 24.6 & 0.937 & 0.066 
& 26.8 & 0.948 & 0.054 \\
Ours & \textbf{31.6}  & \textbf{0.974} & \textbf{0.035}
& 26.6  & 0.956 & \textbf{0.053}
& \textbf{28.3} & \textbf{0.956} & \textbf{0.051} \\
\midrule
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{386} & \multicolumn{3}{c}{387} & \multicolumn{3}{c}{390} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& 29.0 & 0.935 & 0.112 
& 25.7 & 0.924 & 0.107 
& \textbf{27.9} & 0.928 & 0.112 \\
AN~\cite{peng2021animatable} 
& 25.6 & 0.878 & 0.199 
& 21.7 & 0.851 & 0.183
& 26.0 & 0.912 & 0.148 \\
DS~\cite{zhi2022dual} 
& 28.5 & 0.925 & 0.142 
& 25.2 & 0.918 & 0.148 
& 27.0 & 0.916 & 0.153 \\
ARAH~\cite{ARAH:2022:ECCV} 
& 29.2 & 0.934 & 0.105 
& \textbf{26.3} & \textbf{0.934} & 0.088 
& \textbf{27.9} & 0.929 & 0.102 \\
PV~\cite{li2023posevocab} 
& 28.8 & 0.933 & \textbf{0.079} 
& 25.9 & 0.930 & 0.080 
& 27.5 & 0.927 & \textbf{0.078} \\
Ours & \textbf{29.5}  & \textbf{0.939} & 0.090
& \textbf{26.3}  & \textbf{0.934} & \textbf{0.079}
& \textbf{27.9} & \textbf{0.931} & 0.079 \\
\midrule
\multirow{2}{*}{Model} &  \multicolumn{3}{c}{392} & \multicolumn{3}{c}{393} & \multicolumn{3}{c}{394} \\ 
% \cline{2-10}
 & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ \\ 
NB~\cite{peng2021neural} 
& \textbf{29.7} & \textbf{0.949} & 0.101 
& \textbf{27.7} & 0.939 & 0.105 
& 28.7 & 0.942 & 0.098 \\
AN~\cite{peng2021animatable} 
& 28.0 & 0.931 & 0.151 
& 26.1 & 0.916 & 0.151 
& 27.5 & 0.924 & 0.142 \\
DS~\cite{zhi2022dual} 
& 29.2 & 0.942 & 0.126 
& 27.2 & 0.929 & 0.135 
& 28.5 & 0.933 & 0.131 \\
ARAH~\cite{ARAH:2022:ECCV} 
& 29.5 & 0.948 & 0.090 
& \textbf{27.7} & \textbf{0.940} & 0.093 
& 28.9 & \textbf{0.945} & 0.084 \\
PV~\cite{li2023posevocab} 
& 28.6 & 0.942 & 0.072 
& 26.8 & 0.931 & \textbf{0.075} 
& 28.4 & 0.938 & \textbf{0.067} \\
Ours & 29.6  & 0.947 & \textbf{0.071}
& \textbf{27.7}  & 0.938 & 0.077
& \textbf{29.0} & 0.942 & 0.068  \\
\bottomrule[1pt]
\end{tabular}
}
\caption{\textbf{Novel view synthesis quantitative comparison on ZJU-MoCap dataset.} We show the results of each subject.}
\label{table:detail_nv}
\end{table*}

==> tables/secondary_novel_pose_result.tex <==
\begin{table}[htbp]
\centering
\vspace{-3mm}
\resizebox{\linewidth}{!}{
\begin{tabular}{l c c  c  c  c  c c }
\toprule[1pt]
\multirow{2}{*}{Method} & \multirow{2}{*}{Dataset} & \multicolumn{3}{c}{Novel View} & \multicolumn{3}{c}{Novel Pose}\\ 
 && PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow $ \\ 
\midrule
Neural Body &\multirow{5}{*}{\begin{tabular}{@{}c@{}}DeepCap\& \\ DynaCap\end{tabular}}&19.3&0.889&0.129&17.4&0.863&0.151\\
Ani-NeRF &&17.8&0.875&0.154&16.7&0.855&0.164\\
ARAH &&19.5&0.893&0.124&17.8&0.868&0.144\\
PoseVocab &&20.2&0.903&0.105&18.0&0.870&0.121\\
Ours &&\textbf{20.9}&\textbf{0.910}&\textbf{0.100}&\textbf{19.1}&\textbf{0.883}&\textbf{0.117}\\ %\cite{li2023posevocab} 
\midrule
HumanNeRF &\multirow{2}{*}{\begin{tabular}{@{}c@{}}``377'' in \\ ZJU-Mocap\end{tabular}} &30.4&0.974&0.024&23.8&0.936&0.069\\  %\cite{weng_humannerf_2022_cvpr}
Ours  &&\textbf{30.9}&\textbf{0.978}&\textbf{0.023}&\textbf{30.9}&\textbf{0.977}&\textbf{0.023}\\
\midrule
w/o pose. &\multirow{3}{*}{\begin{tabular}{@{}c@{}}``392'' in \\ ZJU-Mocap\end{tabular}} &29.0&0.944&0.073&26.6&0.930&0.083\\
w/o sub. & &29.5&0.946&0.070&26.4&0.928&0.085\\
full  &&\textbf{29.6}&\textbf{0.947}&\textbf{0.068}&\textbf{26.8}&\textbf{0.932}&\textbf{0.080}\\
\bottomrule[1pt]
\end{tabular}
}
 \vspace{-3mm}
\caption{\textbf{More comparison results.} ``w/o pose.'' and ``w/o sub.'' indicate without pose-aware and subject-level features, respectively.}
\label{table:more_quan}
\vspace{-3mm}
\end{table}
